Managing NymBoxes for Identity and Tracking Protection

Despite the attempts of well-designed anonymous communication tools to protect users from tracking or identification, flaws in surrounding software (such as web browsers) and mistakes in configuration may leak the user's identity. We introduce Nymix, an anonymity-centric operating system architecture designed "top-to-bottom" to strengthen identity- and tracking-protection. Nymix's core contribution is OS support for nym-browsing: independent, parallel, and ephemeral web sessions. Each web session, or pseudonym, runs in a unique virtual machine (VM) instance evolving from a common base state with support for long-lived sessions which can be anonymously stored to the cloud, avoiding de-anonymization despite potential confiscation or theft. Nymix allows a user to safely browse the Web using various different transports simultaneously through a pluggable communication model that supports Tor, Dissent, and a private browsing mode. In evaluations, Nymix consumes 600 MB per nymbox and loads within 15 to 25 seconds.

==> todo.tex <==
\xxx{	Major ``big-step'' bullet items for possible improvements
	that might strengthen the story and paper in significant ways:
\begin{itemize}
\item	Explore the full dynamic range of configurations,
	starting from ``lightweight'' anonymization and isolation mechanisms:
	e.g., NAT-based or VPN-based quasi-anonymization (weak pseudonyms);
	Linux container-based virtualization instead of full VMs.

\item	On the stronger side, incorporate system-enforced determinism,
	to ensure that software-exploited VMs cannot exfiltrate
	fingerprinting or staining information from the host
	via timing or other side-channels.

\item	As a step still further, extend vx32 or PIN or something like it
	to do instruction set behavior normalization for the VM,
	so that an attacker hopefully can't even determine exactly
	what type of processor the VM is running on.
	Important step toward making it difficult
	for an attacker to exploit hardware bugs.
	(Unfortunately this still wouldn't guard against sophisticated
	hardware back-doors, but even there it would raise the bar a lot.)

\item	Allow explicit security policies to be bound to Nym-VMs,
	perhaps in the form of IFC security labels with mandated declassifiers.
	For example, some Nym-VMs be wrapped in labels that prevent them
	from communicating with the external world except through
	Tor, Dissent, and/or approved circumvention tools.
	As a more corporate use, some Nym-VMs can be wrapped in labels
	that simply mandate that they can communicate directly
	only with the corporate VPN, and to the rest of the world
	only indirectly via that corporate VPN.
	(The corp VPN is the ``identity protector'' or ``anonymizer''
	in this case - and corps do indeed often want to make their
	employees look anonymous and untrackable outside the corp by default!)
	The corp policy might mandate that certain roles -
	e.g., executives and their staff -
	go through stronger exit policies
	(say, use Tor and only visit HTTPS-enabled sites!),
	to make them harder to track and spear-phish, etc.

\item	Incorporate appropriate use of TPM/late-launch trust functionality
	so that a Nym-VM can only be ``unwrapped'' and decrypted
	by ``approved'' hardware running an ``approved'' VMM
	(e.g., Determinator/CertiKOS).
	Even if the main host OS on the platform is compromised,
	the policiy (e.g., exit through corp VPN and/or Tor/Dissent)
	still gets enforced and the VM contents remain uncompromised.
\end{itemize}
}


